Secrets of Edge-Informed Contrast Maximization for Event-Based Vision

Event cameras capture the motion of intensity gradients (edges) in the image plane in the form of rapid asynchronous events. When accumulated in 2D histograms, these events depict overlays of the edges in motion, consequently obscuring the spatial structure of the generating edges. Contrast maximization (CM) is an optimization framework that can reverse this effect and produce sharp spatial structures that resemble the moving intensity gradients by estimating the motion trajectories of the events. Nonetheless, CM is still an underexplored area of research with avenues for improvement. In this paper, we propose a novel hybrid approach that extends CM from uni-modal (events only) to bi-modal (events and edges). We leverage the underpinning concept that, given a reference time, optimally warped events produce sharp gradients consistent with the moving edge at that time. Specifically, we formalize a correlation-based objective to aid CM and provide key insights into the incorporation of multiscale and multireference techniques. Moreover, our edge-informed CM method yields superior sharpness scores and establishes new state-of-the-art event optical flow benchmarks on the MVSEC, DSEC, and ECD datasets.

==> figures/intro.tex <==
\begin{figure}[!t]
\centering
\includegraphics[width=\columnwidth]{images/intro/eincm_intro_vertical_flipped_3.pdf}
\caption{A visualization of event and edge images (top), and the corresponding
IWEs (bottom) with zero and optimal warps. Events accumulated along optimally
estimated motion trajectories are not only sharp, but also coincident with
edges. The left column of insets shows the edges of a toy pyramid moving to the
left through times $t_0$, $t_\text{mid}$, and $t_1$; however, the zero-warped
IWE is invariant. The right column depicts how integration of optimally warped
events look sharp and move covariantly with the edges.}
\label{fig:intro}
\end{figure}

